A sub-Neptune transiting the young field star HD 18599 at 40 pc

Transiting exoplanets orbiting young nearby stars are ideal laboratories for testing theories of planet formation and evolution. However, to date only a handful of stars with age <1 Gyr have been found to host transiting exoplanets. Here we present the discovery and validation of a sub-Neptune around HD 18599, a young (300 Myr), nearby (d=40 pc) K star. We validate the transiting planet candidate as a bona fide planet using data from the TESS, Spitzer, and Gaia missions, ground-based photometry from IRSF, LCO, PEST, and NGTS, speckle imaging from Gemini, and spectroscopy from CHIRON, NRES, FEROS, and Minerva-Australis. The planet has an orbital period of 4.13 d, and a radius of 2.7Rearth. The RV data yields a 3-sigma mass upper limit of 30.5Mearth which is explained by either a massive companion or the large observed jitter typical for a young star. The brightness of the host star (V~9 mag) makes it conducive to detailed characterization via Doppler mass measurement which will provide a rare view into the interior structure of young planets.

==> tables/tab_transit.tex <==
%%%%%%%%%%%%%%%FITTED
parameter & value & unit & fit/fixed \\ 
\hline 
\multicolumn{4}{c}{\textit{Fitted parameters}} \\ 
\hline 
$R_b / R_\star$ & $0.03165\pm0.00067$ & & fit \\ 
$(R_\star + R_b) / a_b$ & $0.0711\pm0.0087$ & & fit \\ 
$\cos{i_b}$ & $0.040_{-0.017}^{+0.013}$ & & fit \\ 
$T_{0;b}$ & $2458478.71079\pm0.00029$ & $\mathrm{BJD}$& fit \\ 
$P_b$ & $4.137417\pm0.000011$ & $\mathrm{d}$& fit \\ 
$\sqrt{e_b} \cos{\omega_b}$ & $0.0$ & & fixed \\ 
$\sqrt{e_b} \sin{\omega_b}$ & $0.0$ & & fixed \\ 
$D_\mathrm{0; tess}$ & $0.0$ & & fixed \\ 
$q_{1; \mathrm{tess}}$ & $0.37521\pm0.00019$ & & fit \\ 
$q_{2; \mathrm{tess}}$ & $0.28_{-0.15}^{+0.16}$ & & fit \\ 
$q_{1; \mathrm{spitzer}}$ & $0.06800\pm0.00027$ & & fit \\ 
$q_{2; \mathrm{spitzer}}$ & $0.23_{-0.14}^{+0.17}$ & & fit \\ 
$J_{b; \mathrm{tess}}$ & $0.0$ & & fixed \\ 
$J_{b; \mathrm{spitzer}}$ & $0.0$ & & fixed \\ 
$A_{\mathrm{geom}; host; \mathrm{tess}}$ & $0.0$ & & fixed \\ 
$A_{\mathrm{geom}; host; \mathrm{spitzer}}$ & $0.0$ & & fixed \\ 
$A_{\mathrm{geom}; b; \mathrm{tess}}$ & $0.0$ & & fixed \\ 
$A_{\mathrm{geom}; b; \mathrm{spitzer}}$ & $0.0$ & & fixed \\ 
$Grav. dark._{b; \mathrm{tess}}$ & $0.0$ & & fixed \\ 
$Grav. dark._{b; \mathrm{spitzer}}$ & $0.0$ & & fixed \\ 
$\ln{\sigma_\mathrm{tess}}$ & $-7.764\pm0.014$ & $\ln{ \mathrm{rel. flux.} }$& fit \\ 
$\ln{\sigma_\mathrm{spitzer}}$ & $-7.883\pm0.037$ & $\ln{ \mathrm{rel. flux.} }$& fit \\ 
$\mathrm{gp: \ln{\sigma} (tess)}$ & $-5.94_{-0.14}^{+0.17}$ & & fit \\ 
$\mathrm{gp: \ln{\rho} (tess)}$ & $-0.99_{-0.13}^{+0.14}$ & & fit \\ 
$\mathrm{offset; (spitzer)}$ & $-0.000000\pm0.000022$ & & fit \\ 


%%%%%%%%%%%%%%%DERIVED
Parameter & Value & Source \\ 
\hline 
\multicolumn{3}{c}{\textit{Derived parameters}} \\ 
\hline 
Host radius over semi-major axis b; $R_\star/a_\mathrm{b}$ & $0.0689\pm0.0084$ & derived \\ 
Semi-major axis b over host radius; $a_\mathrm{b}/R_\star$ & $14.5_{-1.6}^{+2.0}$ & derived \\ 
Companion radius b over semi-major axis b; $R_\mathrm{b}/a_\mathrm{b}$ & $0.00218\pm0.00031$ & derived \\ 
Inclination b; $i_\mathrm{b}$ (deg) & $87.69_{-0.77}^{+0.98}$ & derived \\ 
Impact parameter b; $b_\mathrm{tra;b}$ & $0.58_{-0.20}^{+0.11}$ & derived \\ 
Total transit duration b; $T_\mathrm{tot;b}$ (h) & $1.856_{-0.020}^{+0.022}$ & derived \\ 
Full-transit duration b; $T_\mathrm{full;b}$ (h) & $1.685_{-0.034}^{+0.028}$ & derived \\ 
Host density from orbit b; $\rho_\mathrm{\star;b}$ (cgs) & $3.37_{-0.99}^{+1.6}$ & derived \\ 
Transit depth (undil.) b; $\delta_\mathrm{tr; undil; b; tess}$ (ppt) & $0.001103_{-0.000037}^{+0.000041}$ & derived \\ 
Transit depth (dil.) b; $\delta_\mathrm{tr; dil; b; tess}$ (ppt) & $0.001103_{-0.000037}^{+0.000041}$ & derived \\ 
Transit depth (undil.) b; $\delta_\mathrm{tr; undil; b; spitzer}$ (ppt) & $0.001042\pm0.000033$ & derived \\ 
Transit depth (dil.) b; $\delta_\mathrm{tr; dil; b; spitzer}$ (ppt) & $0.001042\pm0.000033$ & derived \\ 
Limb darkening; $u_\mathrm{1; tess}$ & $0.35_{-0.18}^{+0.20}$ & derived \\ 
Limb darkening; $u_\mathrm{2; tess}$ & $0.26_{-0.20}^{+0.18}$ & derived \\ 
Limb darkening; $u_\mathrm{1; spitzer}$ & $0.120_{-0.074}^{+0.091}$ & derived \\ 
Limb darkening; $u_\mathrm{2; spitzer}$ & $0.140_{-0.091}^{+0.074}$ & derived \\ 
Combined host density from all orbits; $rho_\mathrm{\star; combined}$ (cgs) & $3.37_{-0.99}^{+1.6}$ & derived \\ 

==> tables/young_planets.tex <==
\begin{tabular}{cccccccc}
\hline
    Name & Cluster/ & Age & Host mass & Planet radius  & Orbital & Reference \\
           & Assoc. & [Myr] & [\msun] & [\rearth] & period [d] & \\
    \hline
    K2-33 b    & Up. Sco M.G. & 5-10 & 0.31$\pm$0.05 & 5.76$\pm$0.62 & 5.43 & \citet{2016DavidK2-33b} \\
    HIP 67522 b & Sco-Cen OB & 15-19 &  1.22$\pm$0.05 & 10.07$\pm$0.47 & 6.95 & \citet{2020RizzutoHIP67522b} \\
    V1298 Tau b & Tau-Aur & 19-27 & 1.10$\pm$0.05 & 10.2$\pm$0.5 & 24.1 & \citet{2019David2019V1298Taub} \\
    Au Mic b & Beta Pic & 19-25 & 0.5$\pm$0.03 & 4.5 & 8.46 & \citet{2020PlavchanAuMic} \\
    TOI-837 b  & IC 2602 & 30-46 & 1.118$\pm$0.059 & 8.63$\pm$1.0 & 8.32 & \citet{2020BoumaTOI837b} \\
    DS Tuc A b & Tuc-Hor & 40-50 & 1.01$\pm$0.06 & 5.70$\pm$0.17	& 8.1 & \citet{2019NewtonDSTucAb} \\
    TOI-942 b  & field & 20-160 & 0.788$\pm$0.037 & 2.74$\pm$0.18 & 4.9 & \citet{2020CarleoTOI942b} \\
    TOI-251 b  & field & 40-320 & 1.036$\pm$0.013 & 2.74$\pm$0.18 & 4.9 & \citet{2021ZhouTOI942b} \\
    TOI-451 b & Psc Eri & 117-133 & 0.950$\pm$0.020 & 1.9 & 1.9 & \citet{2021NewtonTOI451} \\
    % KELT-19A b$^{\ddagger}$ & Lupus & <10 & 1.62$\pm$0.25 & 21$\pm$1.23 & 4.61 & \citet{2018SiverdKELT19Ab} \\ 
    % WASP-152 b & & & & & & \citet{2016SanterneWASP152b} \\
    % Kepler-66 b & & & & & & \citet{2013MeibomKepler66_67} \\
    % Kepler-67 b & & & & & & \citet{2013MeibomKepler66_67} \\
\hline
\end{tabular}
